Anonymising Elderly and Pathological Speech: Voice Conversion Using DDSP and Query-by-Example

Speech anonymisation aims to protect speaker identity by changing personal identifiers in speech while retaining linguistic content. Current methods fail to retain prosody and unique speech patterns found in elderly and pathological speech domains, which is essential for remote health monitoring. To address this gap, we propose a voice conversion-based method (DDSP-QbE) using differentiable digital signal processing and query-by-example. The proposed method, trained with novel losses, aids in disentangling linguistic, prosodic, and domain representations, enabling the model to adapt to uncommon speech patterns. Objective and subjective evaluations show that DDSP-QbE significantly outperforms the voice conversion state-of-the-art concerning intelligibility, prosody, and domain preservation across diverse datasets, pathologies, and speakers while maintaining quality and speaker anonymity. Experts validate domain preservation by analysing twelve clinically pertinent domain attributes.

==> Pics/tables.tex <==
\begin{table*}[!h]
\caption{Objective evaluation. Mean and standard deviation (in brackets) reported. Emo-SG denotes Emo-StarGAN. `All Conv.' includes all conversions. Type column denotes special cases, such as source speaker's domain, source and target same genders (M$\rightarrow$M, F$\rightarrow$F), source and target different genders (M$\rightarrow$F, F$\rightarrow$M) or, `All' including all sub-groups.}
\resizebox{\textwidth}{!}
{
 \begin{tabular}{l|l|lll|lll|lll|lll|lll}
 \toprule
 {\textbf{\specialcell{Source}}} & {\textbf{\specialcell{Type}}} &
 \multicolumn{3}{c|}{\textbf{Domain Pr.} [\%] $\uparrow$}  & \multicolumn{3}{c|}{\textbf{PCC} [$\times 10^{2}$] $\uparrow$} & \multicolumn{3}{c|}{\textbf{pMOS} $\uparrow$} & \multicolumn{3}{c|}{\textbf{CER} [\%] $\downarrow$} & \multicolumn{3}{c}{\textbf{EER} [\%] $\uparrow$} \\ 
\cline{3-17}

{} & {} & {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}\\ 
\midrule
{\textbf{All Conv.}} & {All} & & & &{69.5 (18.9)} & {69.5 (18.4)} &{\textbf{78.7} (17.4)} &{2.75 (0.60)} &{\textbf{3.48} (0.65)} & {\textbf{3.48} (0.49)}&{14.99 (28.09)} &{14.25 (18.89)} &{\textbf{1.04} (2.41)} &48.98 &\textbf{50.37} &50.16\\
 \midrule
 \multirow{5}{*}{\textbf{Dementia}}  & {All}&73.5 &71.8 &\textbf{79.7} &{59.3 (21.3)} &{55.1 (19.5)}  &{\textbf{70.6} (22.0)} &{2.28 (0.6)} &{3.14 (0.59)} &{\textbf{3.24} (0.52)} &{24.8 (25.93)} &{21.27 (20.41)} &{\textbf{2.41} (3.44)} &40.62 &41.47 &\textbf{43.75}
\\
 \cmidrule{2-17}
 & {Dementia}&70.8 &69.9 &\textbf{78.9} &{57.1 (22.0)} & {53.5 (19.9)}  &{\textbf{68.4} (22.9)} &{2.31 (0.58)} &{3.24 (0.53)} &{\textbf{3.29} (0.49)} &{23.36 (25.71)} &{19.09 (18.83)} &{\textbf{2.40} (3.34)}\\ 
 
 & {No-Dementia}&76.2 &73.7 &\textbf{80.5 }&{61.4 (20.4)} &{56.6 (19.1)}  &{\textbf{72.8} (20.9)} &{2.24 (0.61)} &{3.03 (0.63)} &{\textbf{3.20} (0.54)} &{26.24 (26.07)} &{23.44 (21.66)} &{\textbf{2.42} (3.54)}
\\
 \cmidrule{2-17}
  & {Different gender} &71.1 & 66.9&\textbf{73.4} &{58.7 (21.3)} &{54.1 (19.4)}  &{\textbf{69.5} (22.3)} &{2.27 (0.58)} &{3.08 (0.57)} &{\textbf{3.21} (0.53)} &{25.31 (25.54)} &{22.57 (21.13)} &{\textbf{2.43} (3.44)}\\
& {Same gender} &75.9 &76.7 &\textbf{86.0} &{59.8 (21.4)} &{56.1 (19.6)}  &{\textbf{71.7} (21.8)} &{2.29 (0.61)} &{3.19 (0.61)} &{\textbf{3.28} (0.51)} &{24.29 (26.31)} &{19.94 (19.57)} &{\textbf{2.39} (3.45)}\\
 \midrule
 \multirow{8}{*}{\textbf{Stuttering}} & {All}&55.3 &61.3 &\textbf{69.7} &{80.0 (11.7)} &{68.6 (17.9)}  &{\textbf{84.2} (7.4)} &{2.41 (0.63)} &{3.25 (0.53)} &{\textbf{3.33} (0.48)} &{19.07 (28.64)} &{18.22 (20.66)} &{\textbf{0.13} (0.73)} & {\textbf{48.99}} &{47.46}&{48.85}
 \\

\cmidrule{2-17}
%  & {Prolongation}& & & &{81.2 (10.8)} &{69.5 (18.2)}  &{\textbf{85.6 }(7.6)} &{2.41 (0.6)} &{3.25 (0.48)} &{\textbf{3.36} (0.46)} &{18.12 (29.08)} &{17.93 (20.9)} &{\textbf{0.17} (0.83)}
% \\
 
 & {Block} &50.1 &59.7 &\textbf{67.3} &{81.7 (11.9)} &{69.0 (18.0)}  &{\textbf{85.0} (7.3)} &{2.42 (0.6)} &{3.28 (0.53)} &{\textbf{3.39} (0.49)} &{16.55 (28.69)} &{17.26 (21.58)} &{\textbf{0.09} (0.57)}
\\
 
 & {Word Rep.} &70.1 &73.2 &\textbf{76.3} &{78.9 (11.4)} &{70.1 (15.9)}  &{\textbf{83.6} (6.8)} &{2.38 (0.63)} &{3.29 (0.52)} &{\textbf{3.34} (0.46)} &{16.91 (28.2)} &{16.69 (18.2)} &{\textbf{0.15} (0.75)}
\\
 
 & {Sound Rep.}&32.1 &37.8 &\textbf{57.0} &{80.3 (11.7)} &{68.3 (18.6)}  &{\textbf{84.6} (7.3)} &{2.37 (0.70)} &{3.15 (0.58)} &{\textbf{3.22} (0.48)} &{22.5 (28.23)} &{21.02 (22.17)} &{\textbf{0.20} (0.88)}
\\
 
 & {Interjection}&68.9 &74.5 & \textbf{78.2}&{79.1 (12.5)} &{67.0 (18.6)}  &{\textbf{83.6} (7.7)} &{2.47 (0.59)} &{3.28 (0.53)} &{\textbf{3.37} (0.49)} &{20.32 (28.61)} &{17.91 (19.93)} &{\textbf{0.08} (0.55)}
\\
\cmidrule{2-17}
  & {Different gender}&45.7 &55.5 & \textbf{64.6}&{79.9 (11.3)} &{68.7 (17.7)}  &{\textbf{84.5} (7.1)} &{2.40 (0.57)} &{3.21 (0.55)} &{\textbf{3.30} (0.49)} &{20.73 (27.89)} &{19.14 (20.56)} &{\textbf{0.13} (0.72)}
\\
  & {Same gender}& 64.9&67.1 &\textbf{74.8} &{80.0 (12.1)} &{68.6 (18.1)}  &{\textbf{84.0} (7.6)} &{2.42 (0.68)} &{3.28 (0.51)} &{\textbf{3.36} (0.47)} &{17.41 (29.23)} &{17.36 (20.71)} &{\textbf{0.14} (0.73)}
\\
\midrule
\multirow{4}{*}{\textbf{Librispeech}}  & {All} &75.0 &\textbf{77.8} &76.8 &{69.3 (14.7)} &{62.9 (16.5)}  &{\textbf{81.4} (6.4)} &{3.55 (0.57)} &{$\textbf{4.04}^*$ (0.39)} &{3.88 (0.4)} &{1.11 (13.74)} &{3.25 (6.36)} &{\textbf{0.57} (1.47)} &{\textbf{52.29}} & {50.2}&{51.66}
\\
\cmidrule{2-17}
& {Different gender}&\textbf{76.1} &75.8 &75.8 &{69.5 (14.6)} &{63.4 (17.4)}  &{\textbf{81.7} (6.4)} &{3.55 (0.56)} &{$\textbf{4.00}^*$ (0.38)} &{3.87 (0.42)} &{1.91 (14.34)} &{3.43 (6.44)} &{\textbf{0.56} (1.44)}
\\
& {Same gender}&73.9 &\textbf{79.8} &77.8 &{69.1 (14.7)} &{62.5 (15.6)}  &{\textbf{81.1} (6.3)} &{3.56 (0.57)} &{$\textbf{4.09}^*$ (0.4)} &{3.88 (0.38)} &{0.29 (12.99)} &{3.07 (6.27)} &{\textbf{0.58} (1.49)}
\\
 \bottomrule
\end{tabular}
}
\label{tab:objective}
\vspace{-0.75em}
\end{table*}


\begin{table*}[!h]
\caption{Objective evaluation. Mean and standard deviation (in brackets) reported. Emo-SG denotes Emo-StarGAN. `All Conv.' includes all conversions. Type column denotes special cases, such as source speaker's domain, source and target same genders (M$\rightarrow$M, F$\rightarrow$F), source and target different genders (M$\rightarrow$F, F$\rightarrow$M) or, `All' including all sub-groups.}
\resizebox{\textwidth}{!}
{
 \begin{tabular}{l|l|lll|lll|lll|lll|lll}
 \toprule
 {\textbf{\specialcell{Source}}} & {\textbf{\specialcell{Type}}} &
 \multicolumn{3}{c|}{\textbf{Domain Pr.} [\%] $\uparrow$}  & \multicolumn{3}{c|}{\textbf{PCC} [$\times 10^{2}$] $\uparrow$} & \multicolumn{3}{c|}{\textbf{pMOS} $\uparrow$} & \multicolumn{3}{c|}{\textbf{CER} [\%] $\downarrow$} & \multicolumn{3}{c}{\textbf{EER} [\%] $\uparrow$} \\ 
\cline{3-17}

{} & {} & {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}& {\textbf{Emo-SG}} & {\textbf{KNN}} & {\textbf{DDSP}}\\ 
\midrule
{\textbf{All Conv.}} & {All} & & & &{69.5 (18.9)} & {69.5 (18.4)} &{\textbf{78.7} (17.4)} &{2.75 (0.60)} &{\textbf{3.48} (0.65)} & {\textbf{3.48} (0.49)}&{14.99 (28.09)} &{14.25 (18.89)} &{\textbf{1.04} (2.41)} &48.98 &\textbf{50.37} &50.16\\
 \midrule
 \multirow{5}{*}{\textbf{Dementia}}  & {All}&73.5 &71.8 &\textbf{79.7} &{59.3 (21.3)} &{55.1 (19.5)}  &{\textbf{70.6} (22.0)} &{2.28 (0.6)} &{3.14 (0.59)} &{\textbf{3.24} (0.52)} &{24.8 (25.93)} &{21.27 (20.41)} &{\textbf{2.41} (3.44)} &40.62 &41.47 &\textbf{43.75}
\\
 \cmidrule{2-17}
 & {Dementia}&70.8 &69.9 &\textbf{78.9} &{57.1 (22.0)} & {53.5 (19.9)}  &{\textbf{68.4} (22.9)} &{2.31 (0.58)} &{3.24 (0.53)} &{\textbf{3.29} (0.49)} &{23.36 (25.71)} &{19.09 (18.83)} &{\textbf{2.40} (3.34)}\\ 
 
 & {No-Dementia}&76.2 &73.7 &\textbf{80.5 }&{61.4 (20.4)} &{56.6 (19.1)}  &{\textbf{72.8} (20.9)} &{2.24 (0.61)} &{3.03 (0.63)} &{\textbf{3.20} (0.54)} &{26.24 (26.07)} &{23.44 (21.66)} &{\textbf{2.42} (3.54)}
\\
 \cmidrule{2-17}
  & {Different gender} &71.1 & 66.9&\textbf{73.4} &{58.7 (21.3)} &{54.1 (19.4)}  &{\textbf{69.5} (22.3)} &{2.27 (0.58)} &{3.08 (0.57)} &{\textbf{3.21} (0.53)} &{25.31 (25.54)} &{22.57 (21.13)} &{\textbf{2.43} (3.44)}\\
& {Same gender} &75.9 &76.7 &\textbf{86.0} &{59.8 (21.4)} &{56.1 (19.6)}  &{\textbf{71.7} (21.8)} &{2.29 (0.61)} &{3.19 (0.61)} &{\textbf{3.28} (0.51)} &{24.29 (26.31)} &{19.94 (19.57)} &{\textbf{2.39} (3.45)}\\
 \midrule
 \multirow{8}{*}{\textbf{Stuttering}} & {All}&55.3 &61.3 &\textbf{69.7} &{80.0 (11.7)} &{68.6 (17.9)}  &{\textbf{84.2} (7.4)} &{2.41 (0.63)} &{3.25 (0.53)} &{\textbf{3.33} (0.48)} &{19.07 (28.64)} &{18.22 (20.66)} &{\textbf{0.13} (0.73)} & {\textbf{48.99}} &{47.46}&{48.85}
 \\

\cmidrule{2-17}
%  & {Prolongation}& & & &{81.2 (10.8)} &{69.5 (18.2)}  &{\textbf{85.6 }(7.6)} &{2.41 (0.6)} &{3.25 (0.48)} &{\textbf{3.36} (0.46)} &{18.12 (29.08)} &{17.93 (20.9)} &{\textbf{0.17} (0.83)}
% \\
 
 & {Block} &50.1 &59.7 &\textbf{67.3} &{81.7 (11.9)} &{69.0 (18.0)}  &{\textbf{85.0} (7.3)} &{2.42 (0.6)} &{3.28 (0.53)} &{\textbf{3.39} (0.49)} &{16.55 (28.69)} &{17.26 (21.58)} &{\textbf{0.09} (0.57)}
\\
 
 & {Word Rep.} &70.1 &73.2 &\textbf{76.3} &{78.9 (11.4)} &{70.1 (15.9)}  &{\textbf{83.6} (6.8)} &{2.38 (0.63)} &{3.29 (0.52)} &{\textbf{3.34} (0.46)} &{16.91 (28.2)} &{16.69 (18.2)} &{\textbf{0.15} (0.75)}
\\
 
 & {Sound Rep.}&32.1 &37.8 &\textbf{57.0} &{80.3 (11.7)} &{68.3 (18.6)}  &{\textbf{84.6} (7.3)} &{2.37 (0.70)} &{3.15 (0.58)} &{\textbf{3.22} (0.48)} &{22.5 (28.23)} &{21.02 (22.17)} &{\textbf{0.20} (0.88)}
\\
 
 & {Interjection}&68.9 &74.5 & \textbf{78.2}&{79.1 (12.5)} &{67.0 (18.6)}  &{\textbf{83.6} (7.7)} &{2.47 (0.59)} &{3.28 (0.53)} &{\textbf{3.37} (0.49)} &{20.32 (28.61)} &{17.91 (19.93)} &{\textbf{0.08} (0.55)}
\\
\cmidrule{2-17}
  & {Different gender}&45.7 &55.5 & \textbf{64.6}&{79.9 (11.3)} &{68.7 (17.7)}  &{\textbf{84.5} (7.1)} &{2.40 (0.57)} &{3.21 (0.55)} &{\textbf{3.30} (0.49)} &{20.73 (27.89)} &{19.14 (20.56)} &{\textbf{0.13} (0.72)}
\\
  & {Same gender}& 64.9&67.1 &\textbf{74.8} &{80.0 (12.1)} &{68.6 (18.1)}  &{\textbf{84.0} (7.6)} &{2.42 (0.68)} &{3.28 (0.51)} &{\textbf{3.36} (0.47)} &{17.41 (29.23)} &{17.36 (20.71)} &{\textbf{0.14} (0.73)}
\\
\midrule
\multirow{4}{*}{\textbf{Librispeech}}  & {All} &75.0 &\textbf{77.8} &76.8 &{69.3 (14.7)} &{62.9 (16.5)}  &{\textbf{81.4} (6.4)} &{3.55 (0.57)} &{$\textbf{4.04}^*$ (0.39)} &{3.88 (0.4)} &{1.11 (13.74)} &{3.25 (6.36)} &{\textbf{0.57} (1.47)} &{\textbf{52.29}} & {50.2}&{51.66}
\\
\cmidrule{2-17}
& {Different gender}&\textbf{76.1} &75.8 &75.8 &{69.5 (14.6)} &{63.4 (17.4)}  &{\textbf{81.7} (6.4)} &{3.55 (0.56)} &{$\textbf{4.00}^*$ (0.38)} &{3.87 (0.42)} &{1.91 (14.34)} &{3.43 (6.44)} &{\textbf{0.56} (1.44)}
\\
& {Same gender}&73.9 &\textbf{79.8} &77.8 &{69.1 (14.7)} &{62.5 (15.6)}  &{\textbf{81.1} (6.3)} &{3.56 (0.57)} &{$\textbf{4.09}^*$ (0.4)} &{3.88 (0.38)} &{0.29 (12.99)} &{3.07 (6.27)} &{\textbf{0.58} (1.49)}
\\
 \bottomrule
\end{tabular}
}
\label{tab:objective}
\vspace{-0.75em}
\end{table*}










\begin{table*}[!h]
\caption{Objective evaluation. Mean and standard deviation (in brackets) reported. Emo denotes Emo-StarGAN. `All Conv.' includes all conversions. Type column denotes special cases, such as source speaker's domain, source and target gender-groups or, `All' including all sub-groups.}
\resizebox{\textwidth}{!}
{
 \begin{tabular}{l|l|p{2em}p{2em}|ll|ll|ll|p{2em}p{2em}}
 \toprule
 {\textbf{\specialcell{Source}}} & {\textbf{\specialcell{Type}}} &
 \multicolumn{2}{c|}{\textbf{Domain Pr.} [\%] $\uparrow$}  & \multicolumn{2}{c|}{\textbf{PCC} [$\times 10^{2}$] $\uparrow$} & \multicolumn{2}{c|}{\textbf{pMOS} $\uparrow$} & \multicolumn{2}{c|}{\textbf{CER} [\%] $\downarrow$} & \multicolumn{2}{c}{\textbf{EER} [\%] $\uparrow$} \\ 
\cline{3-12}

{} & {} & {\textbf{knn}} & {\textbf{DDSP}} & {\textbf{knn}} & {\textbf{DDSP}}& {\textbf{knn}} & {\textbf{DDSP}}& {\textbf{knn}} & {\textbf{DDSP}}& {\textbf{knn}} & {\textbf{DDSP}}\\ 
\midrule
\multirow{3}{*}{\textbf{All conversions}} & {All} & 71.8& \textbf{79.7}& {69.5 (18.4)} &{\textbf{78.7} (17.4)} &{\textbf{3.48} (0.65)} & {\textbf{3.48} (0.49)}&{14.25 (18.89)} &{\textbf{1.04} (2.41)}  &\textbf{50.37} &50.16\\
 \cmidrule{2-12}
  & {Different gender}& 70.9&\textbf{79.4}  &{54.1 (19.4)}  &{\textbf{69.5} (22.3)} &{3.08 (0.57)} &{\textbf{3.21} (0.53)} &{22.57 (21.13)} &{\textbf{2.43} (3.44)} &- &-
  \\
& {Same gender}  &72.7 &\textbf{80.0} &{56.1 (19.6)}  &{\textbf{71.7} (21.8)}  &{3.19 (0.61)} &{\textbf{3.28} (0.51)}  &{19.94 (19.57)} &{\textbf{2.39} (3.45)} &- &-\\

 \midrule
 \multirow{3}{*}{\textbf{Elderly $\rightarrow$ MS}}  & {All} &71.8 &\textbf{79.7} &{55.1 (19.5)}  &{\textbf{70.6} (22.0)}  &{3.14 (0.59)} &{\textbf{3.24} (0.52)} &{21.27 (20.41)} &{\textbf{2.41} (3.44)}  &41.47 &\textbf{43.75}
\\
 \cmidrule{2-12}
 & {Dementia} &69.9 &\textbf{78.9} & {53.5 (19.9)}  &{\textbf{68.4} (22.9)} &{3.24 (0.53)} &{\textbf{3.29} (0.49)} &{19.09 (18.83)} &{\textbf{2.40} (3.34)} &- &-\\ 
 
 & {Healthy}&73.7 &\textbf{80.5 }&{56.6 (19.1)}  &{\textbf{72.8} (20.9)}  &{3.03 (0.63)} &{\textbf{3.20} (0.54)}  &{23.44 (21.66)} &{\textbf{2.42} (3.54)} &- &-
\\
%  \cmidrule{2-12}
%   & {Different gender}& 66.9&\textbf{73.4}  &{54.1 (19.4)}  &{\textbf{69.5} (22.3)} &{3.08 (0.57)} &{\textbf{3.21} (0.53)} &{22.57 (21.13)} &{\textbf{2.43} (3.44)} &- &-
%   \\
% & {Same gender}  &76.7 &\textbf{86.0} &{56.1 (19.6)}  &{\textbf{71.7} (21.8)}  &{3.19 (0.61)} &{\textbf{3.28} (0.51)}  &{19.94 (19.57)} &{\textbf{2.39} (3.45)} &- &-\\
 \midrule
 \multirow{6}{*}{\textbf{Stuttering $\rightarrow$ MS}} & {All} &61.3 &\textbf{69.7} &{68.6 (17.9)}  &{\textbf{84.2} (7.4)} &{3.25 (0.53)} &{\textbf{3.33} (0.48)} &{18.22 (20.66)} &{\textbf{0.13} (0.73)} &{47.46}&{48.85}
 \\

\cmidrule{2-12}
 
 & {Block} &59.7 &\textbf{67.3}  &{69.0 (18.0)}  &{\textbf{85.0} (7.3)} &{3.28 (0.53)} &{\textbf{3.39} (0.49)} &{17.26 (21.58)} &{\textbf{0.09} (0.57)}&- &-
\\
 
 & {Word Repetition} &73.2 &\textbf{76.3} &{70.1 (15.9)}  &{\textbf{83.6} (6.8)} &{3.29 (0.52)} &{\textbf{3.34} (0.46)} &{16.69 (18.2)} &{\textbf{0.15} (0.75)}&- &-
\\
 
 & {Sound Repetition} &37.8 &\textbf{57.0} &{68.3 (18.6)}  &{\textbf{84.6} (7.3)} &{3.15 (0.58)} &{\textbf{3.22} (0.48)}  &{21.02 (22.17)} &{\textbf{0.20} (0.88)}&- &-
\\
 
 & {Interjection} &74.5 & \textbf{78.2} &{67.0 (18.6)}  &{\textbf{83.6} (7.7)}  &{3.28 (0.53)} &{\textbf{3.37} (0.49)} &{17.91 (19.93)} &{\textbf{0.08} (0.55)}&- &-
\\
% \cmidrule{2-12}
%   & {Different gender} &55.5 & \textbf{64.6} &{68.7 (17.7)}  &{\textbf{84.5} (7.1)}  &{3.21 (0.55)} &{\textbf{3.30} (0.49)} &{19.14 (20.56)} &{\textbf{0.13} (0.72)}&- &-
% \\
%   & {Same gender} &67.1 &\textbf{74.8} &{80.0 (12.1)}   &{\textbf{84.0} (7.6)}  &{3.28 (0.51)} &{\textbf{3.36} (0.47)}  &{17.36 (20.71)} &{\textbf{0.14} (0.73)}&- &-
% \\
\midrule
\multirow{1}{*}{\textbf{MS $\rightarrow$ MS}}  & {All}  &\textbf{77.8} &76.8  &{62.9 (16.5)}  &{\textbf{81.4} (6.4)} &{$\textbf{4.04}^*$ (0.39)} &{3.88 (0.4)} &{3.25 (6.36)} &{\textbf{0.57} (1.47)}  & {50.2}&{\textbf{51.66}}
%\\
% \cmidrule{2-12}
% & {Different gender} &75.8 &75.8 &{63.4 (17.4)}  &{\textbf{81.7} (6.4)} &{$\textbf{4.00}^*$ (0.38)} &{3.87 (0.42)} &{3.43 (6.44)} &{\textbf{0.56} (1.44)}&- &-
% \\
% & {Same gender} &\textbf{79.8} &77.8  &{62.5 (15.6)}  &{\textbf{81.1} (6.3)}  &{$\textbf{4.09}^*$ (0.4)} &{3.88 (0.38)}  &{3.07 (6.27)} &{\textbf{0.58} (1.49)}&- &-
\\
 \bottomrule
\end{tabular}
}
\label{tab:objective}
\vspace{-0.75em}
\end{table*}

==> diagram.tex <==
https://viewer.diagrams.net/?tags=%7B%7D&highlight=0000ff&edit=_blank&layers=1&nav=1#R7V1bc%2BM2lv41rso8CIX75dFOpye120n3TqcnybykaIm2lZZFRZLT9vz6BSiSIkHwKlKkZboSt0VRAHXOh3PHwRX5%2FvH5n1tv8%2FBTsPBXVxgunq%2FIuyuMEcNM%2F2OuvByu0PjC%2FXa5iG46Xvi8%2FK8fXYTR1aflwt9lbtwHwWq%2F3GQvzoP12p%2FvM9e87Tb4lr3tLlhlZ914937uwue5t8pf%2FXW52D8crkoGj9d%2F9Jf3D%2FHMCEbvPHrxzdGF3YO3CL6lLpEfrsj32yDYH%2F56fP7eXxnixXQ5fO59wbvJg2399b7OB758ZH9snrb%2F%2Bb%2BvEP8%2B%2F%2Fhh%2FyF4nhFyGOZvb%2FUUfeMr9kP0wPuXmAp7%2F1nPcfOwf1zpC0j%2Fudtvg6%2F%2B98Eq2Oor62Ct77y5W65W1iVvtbxf65dz%2FZS%2Bvn7zt7%2FdLzV9r6M3HpeLhZnm5tvDcu9%2F3nhzM%2Bc3jSZ9bRs8rRe%2B%2BQLQDB%2Bs9xFCpH6ZJ0BEEzOF%2F5y6FBHkn37w6O%2B3L%2FqW6F3K5eEjLzH7BIgB%2Bu3IbhxR6SHNaQaiG70IYvfJ8Ecu6D8iRriZ8pckH%2FcK%2Fevnm4%2Fqly%2B%2Fedcz9DwTeZ7YDLnXlNnUJ0CyPrzbeARYShiMVZYwHOeowmGeKgT2RBN%2BSTgt5Xpt8AoLumeErVOWIOFgEuarfUSSDKv4X09G8N1k%2FrqP%2Fg0%2Fstt4a%2BdHzFizXUjfa30Dgptn50DP8Uj62xwGsyZ4um34SIXfwnokCYj%2BKXiszUOwTj3ZYczsPOaBzcPlrmZvfpPgj%2BAuzyaOnFinEDfHuo2SAoC8hxfG8RZq2dI%2BGAGHVkaJrs5IONoTz%2BOHOoHlqEgo%2FKHfLPm%2FLRzqs3nr66eMrAPD1E2wXO9DCrKbK%2FbOjPW0Dw7fpBHSukcHoiiDDklz0EDonMKgjd6bgGEBYxvsvf0yMHPPkIRdQYWMCyqJHd2D3vg52D5qvu60YMZwUiKI0QzvVV6DCJeB3B%2Fri8XExsn31XLtz%2BJnO0gJ%2FXAsJA%2BsCYquwPX5abP1Zjv%2F%2FlFzxNNflnuPhovr292m2Ea98739k5Ygqbc3bw%2BIKAtEBLlDCjktmR59NeYAo8WQLGFcpEvxyqJbmktXmPgL%2F%2B6OFbF04e0ewnlQ9OKTt9eMXIdXsDa1O%2BHDjFhWJclrAywd2gAhfjobbr9%2B%2Fu%2Fm193ee5qvl3%2F9eSPll%2FWM1Qj16GGWm10ReNMcyC%2BMLLU1HxZC3UJok7wTkOMscUU%2BYIRcAQkqe6ItgjUgXpu43m5zCC%2FfLZ8N3bqgGaEiXuAx1ShyxR%2BdwqEv0VCipmpbs5Uhmfqxl802eBNhkcbowcRyg0QON32FRNyyjFYvt%2FKwtTtG3VAKgTgykywpCZhjSWEBqMqTR1FAe1O6rD%2Fj%2Fxu6sPVQjrH6qwQDLhiVBGoTi2sNZNliGCAKCeSYU72CYgalgSIAp5pzHEmBpBLxI2RksUad%2FiHQJJSUvq03ALnWWEcAIhOAXABiHECkWQqFEJArziyNjQ4AglrQKCihI8KACWBalhGqtPfP9K38LAhyfn9XvtctpK2IDGtO4w7EOQREKCmVUlQiJLPBHIKB0KSnjEmm6eqgPNfMYQIrKKRmpP6VJzzDAEPtWOv7qGai6CB47CSKy6jqzBY9rL%2B4PgECw6yNv13qR%2Fe3Zpzl%2Bj5aNmE4L7kVJVeSIgbk4rzlzd3d%2BXw%2BL%2FUvamIlwWN9ga6AUkQzlQspEYMsm8GHhp0QSa32EdFSX4q8s02BgJTqxSwJZpBDl3mtzQDEFaEagwgKFXsuneOiSwdwWFxoD997Ohj3A6BCAsIQYYJrMYEE5VlRgRGgGfmat5XHBIo4BnkBqNDcfx%2F%2BDIMLjrU5r7TdhLRXqhKnOYYFC7Wu0IahwBQrRsYNCzTBohtYSAiQtsOkFgiCSKSynrQ2%2BaWGhbYIuEKQcpq3LEYFC5dXOcGiBSyoclvqcQYpVCKEa9sDC85RvgZlVLCoYepPsKgDCyG0oyGp4Nre1LoiTuEePUAjLSjWnghnHI5didQI002wqAMLxoH2KTllRCGEpaVECAFcw0Ip7YoIbiIH44bF5KB2BAukgOYm054nVpBrzmbFBQYc5wM9Y0XF5binQ5sWCGgRQbRHohjTFmUuiviqdIicYNERLARAhqWIanmgDQ1bhRiDU3GhtJMKlcinsUaFCld97ISKNpaFFgdCCwNJoZBCWolexEPLglHzg6jC47Ys8BTM6kpYUCCR0GJCEZNwopZ7GgU5OWeUIEHEyC1OPEWzuhIXFGi7QssCqRSDhEMryilCXEjE9Q%2FGrkTZqHAxhbO6Cn4beZFKiljWRZj5hIoIzohEmI0cFlM46yzhLILCnIiCwjAejR0VUzSrKyUigSJQUiklFoxiS4m8NqOz19rft5NXJwIoVZg%2FRQow%2FbaCCrMQPONOq%2BOLinEOKSzCcotUpixrb6owmCWFQNyU4oxdVEwxzq4MC1RabCGNG4IQUtokRYrxkQuLKcbZlRuitYS2NLnGBjM1F1bUAhp7E0EmubYrIBp35BtPMc6uhIW2NzFlQjKOGE%2FsyUxl1mtBBbmoEOeQyVNOAVEp3zQb%2BZ5xoG1OpYgRJNpDcTSlGhUsJue0o00YSjOeMIIEJcZ6yNmbyuwDkBwqRQlz7PYaFSomw6IjVCAIgZYFAlNqwtrMrsBhIS44EYSQozk6UljQi9Ihg8IChSYlJgQxRLWHmvVDGAKMQ0ogFpxxpsYd4KRTlqwjWEgMkPY2FKdSEUmyoCAEMC0rtJcitbWJHc0LRgUKPIGiI8MCa7YKaIChOSes3cFEAmI0iBISC4GYGjcqpgxZV6iQQBsTFCkkqaJCZROnjAGkFQimJuIlOcs3Xh0VKiYnpDNzkwCsmMQcafdUSZaFBQ3tCqIRo31TLU7GXdlLLydBNrSwML6pcS8020x9b9awoBQQjQolIKRKKDhyJ2TKkHUmLKR2QigiiELGiY0KDJSEFCotU0yl3sjNzSno3aFrShimhHPtgApqlWRRGAoLiUxnAwLpuBOnbHJNOxMWVBucWg4gzJCizOoxow1O7ZxSU8MnpPZWRmNZFDQpcvkhHTUpwq%2B6SVEKg73iiUqtXignQqsfwYjV9xKjbM%2Brls0wVFgQps1eZYYQtIPOOe5W%2B87Kz2Z9c1HjvrmfgsA8WXCnf3160MjQENB%2Fvk8a2sK7bfB4hZM2y0lfwl9SEE03Kyzql%2FvqG%2BJ2BNqZKROAqZ%2BsEBRafjm6dxORRyaC%2FfXNreVOrxfX5ugpw4CVt9st51kuZunrUnT%2B83L%2FW%2FiKchy9%2Fj18LVX08t1z9PnwxUv8Yh2foUXzrNMc2778ltypX%2FyefnEcMXz1khr%2FU6x4CyVXZAvsgqft3C%2FVDpFRs%2Fe2935p8jhKiPiLzAldefyk4MAcDS%2Fja1t%2FpYXv337meV0AiWb4ZBrdp3Q0y1YoIG5h7PDVo08dYZYfyAonYWhJzgNlcgOFeE2%2B9ikQrhM9bgThErgKVBOvDlFzxOthUdRFbHZF4fCKt92nJhoK0%2FxCIS1gdiBl9S%2FsG9KiTg3nCVKZZEEueCOQdwTr7Fr58%2Blxk3o5FoSjS4U4sY5bk71B%2FN2v8KMvfrjB13%2FeBj%2F%2Bsf3yH%2F9mVsPXvrB2%2FVRlk3EK5q0%2F5Gqlyvs7weNkT%2BR4gEdfB3V8CJ4Wa3%2B3K3SUL8fxaH5IgXWumMxH410t03s8MpHVKQZrpLgsquX0QqJEeF6JFJJ4LNIcZ%2B0MZY1QW5gzy16BVjCsQJhrNngvqduis7BqP288zxEyhxE7NYYodGGqWbwEn3rO0DzRJccbyV34k%2F%2Fsr97fH36qOhniNtgu%2FO0sGvg6%2FH7b72az9PV%2FOB%2BNNzw%2FIornbE%2BRwrXE7HHhosYKOxelPsRM8qo8ud6B%2FLS66oZHK%2BQkKHHEClFfweY6zUUuzC7CwupK6bCLlIsH%2FdlFdQqPmgUU2rpIkY8W%2B2MH%2FwzHIbVa7tnYlSAhFv8FQLilV0MYBemQq92WjFqQ6UgvEvtoPtG%2FWqzV97ITkKJWIL0sjGJLUygGRGuMslKMsnqOeHOM2nvdWf8gJXV2AewevI35c%2F6iDTdt%2B5BqrXZ7AO6H2%2BSCN%2F96H8L549Pe2H%2FR9fgcV9aL%2F5Vsqi05JM5lPrC%2B%2FC%2FXDq3v31%2BZ2E65NVrTDHwoNz0Lj7i%2F1c%2BmRw9LHMz4kZGrLx%2BM8pQVvN96613MlfC9p%2B0uefPgyBu%2BBbvlIfVsrnu3u2D1tPcP74VD3AXbx1mwXd4vo3vMGW6H34eb9FCzyL2%2FDh9aO5aHt45gSpvn2%2Fvb70LOfW9sn9QfBysdrvy7yN2QEAOscDJTsIncECUBVzy%2BXkDzw%2FU773G5eokeTX%2Bd2c7fLu8spsDFMuuUrPbbzPvbwGLEZuvvzIGnIenK2Rvy8o0FVKjtSJP8gu7rEDr3gnYlAroJrHUqGNatfNJJXjSWFyVyoTq00bW86AqKDxU4mcRR7L%2Fkd%2BycVRy5sjbNInGwMBJXeMiqO%2FZ0uLZY%2Fl0HeKroFPBDojAVIqs3vC0MEvgUP32xrHNKj%2BVaiytv5Rzyu9%2F%2BUbgyksvho9e5mqOpi84VN3W%2BHg%2FC8ZTVGJiS2r1ZOKifxTmzNtcp5Agexjm%2F86xOl7PVjYT%2BtA12wcJ8%2Bx%2FW80Dr4sNfGeuh5vnG%2BVVWVft6Sly5A0bj%2BJzFmNHUwWguHYwmPSba6vvVy0fPBFHSRLLXVWhyJFc%2FeLf%2B6lNiML27Dfb74NGIc%2FPGTSKvMj1WwlQIuQknu46L383Ky1XCR8%2Fz7mG%2F3%2BxC2L3X%2F80XawyW82B9FwYBwNxUo75feHtP%2F2Ou7%2FS%2Fnolm7WaelpVP66V%2B3p23mnlz85y7mblJm0MaR%2B%2BxKZN4v1k97f6YL7fzlT9DWIKNMSd7AAihVlEGdYSwHfjo71xd1waXjo48T5ZxfAEDffv7p93BQnRVCr%2FeAvcuwKGycTdM8jacchT99oWN06vP1anJ1PZaKNjtZ9f7veZGiDb4s3baNPt3sX%2FSukKkkYpJbXtQPYFGwiS%2BnIQiFHAcmBFHHM8iV2o1HG1VadtH7qBGFeDVqJIMViE1itVK4wyDsAdS2YF6Ll%2BVncPErjhNSlcZzNZnY1wKHVcVacEugmMOrCDt1R53hEYLNF19WmrRjwSh5og4q7EhgmYzH1XHn3aYxdIKdSDr6fouuXZWGVmgjU%2BSt6ooFp4v75wNBvlc%2Brd3p6iIomPni2sCbb2B6sWMUH9eKa6mbNPdtJX0rGBytSZO2%2B7nJVeN6pPxkes5S5bhqFejLGK01MODU69GWGG01CODU6%2BG3TNa6rliFuelXo09T6OlHhuaenWOsHwV5kvchSMph8pT9rzmS51jIBvjsnsOVMBixAYPc4nNjmocjsHK9oP89QbCmiejJ06KZXNiM5wXi65AeF%2B9NlCdevoTlUrNs42Sldwf8Qc3vuscgXkx1B7cWI%2BJ%2ByaoPbhxX%2Be8xouh9uDOQJ1zEC%2BG2oM7D842mQ3ruvreB%2F7FbD3z1nPTq6qw91SzItPGhVdh96xfDkF7DD9vfO9rWAmTy4kX9cyqqNkad0VVHyVUVie3OOudXgnCUUIV%2B2Q9OCN1%2Bgi33FZ11Si%2FVJjzMjmWTLYUx%2B1c6ie9CplXnTSN8wuVrVPEuPZwJUot6VNlydPaqSrBMxu4sDUstau%2B%2Bk5d8RpOzjjT8k7cxM2WRoIblZVR2hBsvfUv16fB3ufaO1I67ytVryVf%2B2R6pZQZGVrsUkB7hLpQ4e2Q0nRXaO5xz7ApFDdKtZ8t8jzLrnPlOKJRAZX5cRgmoi%2FDRNXwiGoTrYIvJ9NSy0hIBUcq%2Fp3vdIo5UMwUusW%2FHcTk4DiC%2Fi15X8SVzTbTR6Z1XaFYk%2F4Ji0ciypA5%2Flgo02%2BZaq3HYctytKJxXupxuW%2Bd2LBa7Y3wngGFmIJcSImpyDW8qW%2FxuMcZC%2B%2Bb2UNvhPcSIEqlJFQyAhVEbdd9wThn573bO60Rzz3o04ZcdKvKRkdJZ%2BiEAUFYYYYENKeNY8c580hV61JzmhPlmEkGyfEA6h5UKT7vkipl7tArKj4HBaQIzyFr3N4otknBEQZalkLL2OxdWjbri3XZrI0tXYCIkkhwrJBQhIiGnC0fJqnhLV28vfO9WUz0TfCdA6aEEMgcywuxolm7pkhmN44ClM4ytDho1uv1TcACEUAEkRxqPUgEtHYOdwWL8lmGhkWd09XeGiwoYFrzCyERYgzaXdw7w0X5NAMDQzVLU7wNYHAgCZLInNRNFaXW7qqTDcd603CgiBSCMa1oYNJv%2BWy4qHPu3lvDhfaduUJKMUUFQQz2hIvyaQbGxeRJOg5bcnr6XcOidJaBUVEjXDuaPEjWjYPgSNHwtyMrAkeUFVHjiI6O6wQeAqjCkJP4NyoVmaLlduiKWXIBAauAvvdFeGbX71UggwFOzEnHCCNMscRWbVtHNn75LNozTItmxM5t45%2FZ%2BXsVwBBapkOIuJRaWgvUju%2FOQcaRRksq6Saup40oCKBUklCGWHg%2Bermt1jbBWj7LwIoCwzP7dq8DGRgYy0BALCFBUNiBmNq8LxhnLFLhzP7b6%2BC9XveEK8qVEERg1lIbFAwzFs6fOVH4OjjPgeRMYcIFpYQSqxSmK31QPsvg%2BmAchXYjQ4YCEDJBEYGEa%2BZT0QsyymcZHBlTsMFRFuAOB3UbayifZNikUVKG3QwWmZPrUhjJH2JHrlznq1tYynbruLvz%2BdzZrWMh1C10oM%2FdbjmPyXFtmJohnEFCEs5sCrDcQOcGkbMx%2Bgmy5VQ8jJ7z2LInJQRYMoFo%2FLslEHLjEnAc0%2Fw%2BMy469k4vHhdIalWhDUutDKTWOjzb7QUJATLcxG3lRfk0koI0FmsemNcdajr2ay8fNRykmEkksXwS0bLAvHLgc%2Fu9DQ%2BOnZCBKBBQLyihXdZwwVvRSyFBRu20BkrFPEProY694svHDQZUKu3GRly1sqPtBUr5uGeXJx0XXl8%2BLiA4Ms8s9c6AUTHw2ZHR8abFi0eGBJhQSDFjBClEpQ2MjhRNxTRD65mOY2wXjxqTR0EpjdCTeVIxzdCo6bjY5%2BJRQ4ASUqQEgc3PjqIplfMgkHaT46OCzoabjmuBLh43OOukCGy7s11F4armGRY3dXr2TrhJG6f9wMQedlhU0EmaNJQmLLvM4zBpkoRh3RgvVfNo12lI64VN0qQhbkhZDCSp7WmOk%2FJxz7ypPSmZmnBRFxeoNARyAjAqBj47MvCEjGb2hyqNenSmaarmGVrTTNmfhrgRpXGP7nBTMc%2FQuJmyPw1xQ7OBD2zBRnTk%2F1RMIwf1hxo2Kp9Qg4gd9ugJNlXzDIybKXPUEDd94WRkuJii%2FA1xYR8nwDvChT2uGtY6meJuzXAhsrWLObOBdFMjWTGNtmmHrJFseCTFhBpWWsmY7KVsDJOKcRE%2BMy6mqFszXJDSwkVz2EwnLnLVNMPqII4n1DSzTbKhdqasltKtxUnVwGeXJ1PMrREyINBKAB%2FDGsQO1bYERtW4Z8fFFFNrhAsMEtEf2grUgkU3aqZqloG1zBRRa4QZjYnYrAxXfj%2BmSdUsw2JGTH5OQ8skWx2CFO4oamKPy4bFxeTnNMQFs%2BIZVl87qTraWloxj%2BKDxk3iqO%2BEm7q4IRVbQE9J45QNrM6NjMnTaYgMVFqXiBTsqLqgap6BNdGU72uGm%2FIio85gUzXNwKiZdoo1Q015iVFnqKmaZmDUTDnkZqihFTu4uvKOKuchg9YeiCnH3Aw3uRIj2zjtCDeV8wyLGzlFX5rhBvcDE3vYQVFBSDMtNF95u91yXgYMzc7ty2%2FpF7%2BbF4DFL989p9989xK%2Fel7uw48BpVj0%2BvBJqg2sw%2BvjR82L9Cc%2F%2BdulJoa%2FjeFZE2wHtpVRiEZwOnCi5E4K1agAHDclPaarAG5pShGsmXL8EXaG9LybTghppgJ7BO0rk2l2w3vW8swjTsrH6RsAcUSzOwC8MkbaR9zA1mfdZceh52Zks0BdnZUcqRGUUSGsVIF0pizGpgJ4hdxue1i9VXZ77vguoc0qFpoogBkESLtYGS3AVYUaCF9VmCBtgDl2MaSs8G1bfYIoBUJImPxge1zA%2BfHdc9sb1BUW5qt9xOQM7vhfT8E%2BZF3qr3vz70v8md3Tbc2PVM5i3pjtQpBd6xvE5tk5zkM8kP7%2Bh7Gy4%2BvL4UPlrmZvtlbY3n%2FeZ9dU1vmLXMi0pxhd8qLe3nONa7Neck2%2FH5eLhZnm5tvDcu9%2F3nih2P229TatNXfugML8onmOF4cFa7NbIUJ2al1xx7oisHgJnXS%2BIKGuIPNrwuBuwuApGBQIiMExWCNYEFPxg3frrz4Fu%2BV%2BGRhq3gb7ffBo%2BPPgLUKtbAiXnD0AXRxJcdV9KkD2MAJ0GH1jnuTx%2BV4z6gE8BvOvTxvw6G3NP%2FOn7erlZhty0snWXPTqYDiFDN970VdR%2FbDcnFFBbMmDABE5rhOVyKM043FvjHf2%2F2gmFhAskAvxQMnSR0Df%2FunBrFIMf%2FI2G42FozSYJET8LrO2p8RRkRRQ4tRZGiWyL5BIly934NHGiZDVcu3P4kcLMWJibSwkD6wLn%2B%2BDtabZzqzMGEjb%2BL3fUxjZjBwggX5zuTe8RD1pFJaNByKCXFZNvIXxPBpFusqIG2FGFEJGVgicupKraJzP%2Fupudr3fa5ak0Fds3RQj8IgEVICVjN%2FatyIiVAFLD2mNEx8ulMJKnKzInLgtgb1%2FoUO4NKvPGThcNBInndgJbM3eln46ta3S%2FFB9%2B%2BKyWbHNBIGQb9iK87Y9SpPaJcD2QL2z3%2BWCvBKF8UE%2Fire9IEVBEQLSOhlRa4qYR9WaArNiJJ%2BmKVSzaocGYsI0jJUZUQEFLRUWx%2BQiIEhepULLCECErrqJLdu3FPK3OuUdM3As0ss%2BsZe07J5IlQJcIRaHke3zXgkBCLLj25Yd07dsU832wTTCLKPZmgqIyhVcCrOM2pjFZMJsU8y21rgas9ogT0CZ1%2BSA0mPm5NyQxV1D1kbJEYeCdyM7j4tCCEuQQ1W%2BKC4cslaAgLc8I7dKzHIJlMLHtPR5C6%2BJKs6kjN6EzAVL3737%2FEnf%2F%2FllvX%2Fwd8tdw1jpK7Q5Bc1FyYl0RcmFSjImmSi5tF3WDq3OHqspj7Vov2dk3UUUpjFs%2BZVtj09mlINUoQC0Qx%2F1ZI1mkPeSum1jbtiVPD7lzsc%2FgukwYseCrMcyyCzaqvTsa0ebtMymjtDGrWH7Qlv0%2BL2ijcLevJMLDrwxZlfctnRdGbdLrc5bA5VUNp6Q3cOnmk3zJC9%2FvJHchT%2F5z%2F7q%2Ff3hp6pyl9tgu%2FC3s2jg6%2FD7bb%2BbzdLX%2F%2BF8NN6wbuWYmzzd%2BuvOXrN28Ryk2JWjDiJ5p4e6B8vtiH3KdMGDI49tn3TRxop79yv86IsfbvD1n7fBj39sv%2FzHv4k36Jyl1oGAE4x3i%2FHjyGP3kLi2%2B3C6bH2RB4g6HR90%2Be%2Bn%2F73mqz%2FV%2F2yW%2F353vfjl%2BXbWTA9W7aMbuwbLWbZt41jZcZQ1THfq6%2Fbr5%2F9uft3tvaf5evnXnzdSflnParU%2BXK2Wm10RylMM9HYbf26ofLd8Nny0ytAOJswmjhOZcZbr%2B4jdW9%2BIiXTF2uHKjzHnLC96FsZpLTH9Pvxxielks2UH6w5pTxkjwZBQWEhELTltenhzBSkyN1Kz7TW3Ks1B8pRCriTRcOQQOdxxCijiilBT6wb1TB1IdTcC6mwZmBBgIUAAQqAgUgrBOId2o2UEpEaACTsrzqXIy%2BVRIaBOy8LXgYCFf%2Bc9HQzbfvmPAVGawxSZaG4ScEh3LVSQEM4QQpKOm%2F3OLnPdRGXDYlVtMOlbfljPg8XRjiuw99u7HXr8%2FnyazUOmjs3h1hxrK%2Btapc3cke6dC2klH0S%2BOCF2rTMlj6SLKLEbiDU00b0m26YBQebBeq3lkXcbDwCbEmoWfyQJlTqWs8psJ4zFQcYrE31RrYb0rk21Ur6cTktMAKSCIxX%2FpjlSYg4Uw0TC%2BLeDlOak%2B9Q4dh%2Bk7kjbcdezdtSPKDAStwchQJlQ2vdU2sIlvP1WWfc4L%2FV43LNb1HXnsovgPAMKMQW5kBJTkYsz1eZ8wTgj4XzH3ccugvMSIEqlJFQyAhVEbdd8wTgj4XyNrOFBkTZj4ulq0%2BpOAAjCCjMkIOQSYp63R5CqVqIIME45ZpJBQmEXQWMnFbrurtVuPY2k%2B8RL7Nml6M4hs6t9K9dTHCsERxRoOQotE7Pn9SI77k7%2BqjkbG7gAESWR4FghoQhpWaxRMEwsJ8uXbt9sxxPbc%2B1kAFNCCAS1ewyxolY4sEBgN24uVTrLwMKg48bil4AKRAARRHKIJCYCxgunY1SUzzIwKpq1I3obqKCAaa0vhESIMYgY7wcW5dMMjIuOD0m6CFxwIAmSiDDBqaL2zsSTbcZ603CgiMlpMa1lYLKr9VywGEW8bWSw0D4zV0gppqggiMGeYFE%2BzbCwGEUwbmSwcHv4XaOidJZhQVEjTjeWtEfWfYPgSM%2FwtyMJAseTBJEdt9VvxYuR7QgjgCoMOYl%2Fo1JpGYuOxs2ly2fJhQF62y7mZEnDjeRvAhcMcG1baYsbI0yxtHZTdGXal8%2Bi%2FcG0UEbsvKZ9w73abwIWAphtyohLqeW0QO247hxkHJmThpud3wTPEQRQKkkoQ4xwTkm5hdY2l1o%2By9AqYgxBwbHhAgNjEQiIJSQICjvyUpvzBeOMRCKMIfA3Ns7rNU%2B4olwJQQRu2%2FeiYJiR8H0Mgb2x8Z0DyZnChAtKCSVWvUtXmqB8lqE1wRgie2PDhQIQMkERgYRr1lPRCy7KZxkaF2MI7Y0MFwXBn25jC%2BWTDJsdcjYLabujur%2Bd0xtv7Xwaa28EB1z%2FFDX%2Fz%2BxZiNp84%2FKtBuZqOPfr3FidXaIl%2B6kLdmDnF3XjvQ%2F2KV0o6XyT3lrtCrr2VSWHYA2DOW7hv3z07i0x6D4FoPLIgZV548abf70PeZg5tjJcAuQmnOw63tQVnkZg7%2FCKnufdw36%2F2YV4eq%2F%2Fmy%2FWGCznwfpuqdGxBXM9I36%2F8Pae%2Fsdc3%2Bl%2FPSPYdzNvvZg9rZemX7m3mnlz85y7mblptvM1pN9jk75%2Bv1k97f6YL7fzlT8zmzA3ZudYLxurBbDtJ0pA3LUkXWjp2CGDOmgkXwCSzrs8v7KuITIb6rT3StevQIel43TUjsa9s7voodzfravWNQWAqmF%2BNd3v2cOBDtyOauUPdEAO0MXXeliINZKPI6Cb3WPnjHT7S5KPe4X%2B9fPNR%2FXLl9%2B86xl6nqEa8cCCCvuiL1%2BUni0mCs2ufRQXwJzh8CA3UVyav%2FH5VU2t0sJOLM8VZmZ%2F52NJQPRPwWNZO3Df3DlZ5eupWiR0j279chsYHh01kjlY6qdg4Zs7%2Fh8%3D
